Domain Adaptation of Majority Votes via Perturbed Variation-based Label Transfer

We tackle the PAC-Bayesian Domain Adaptation (DA) problem. This arrives when one desires to learn, from a source distribution, a good weighted majority vote (over a set of classifiers) on a different target distribution. In this context, the disagreement between classifiers is known crucial to control. In non-DA supervised setting, a theoretical bound - the C-bound - involves this disagreement and leads to a majority vote learning algorithm: MinCq. In this work, we extend MinCq to DA by taking advantage of an elegant divergence between distribution called the Perturbed Varation (PV). Firstly, justified by a new formulation of the C-bound, we provide to MinCq a target sample labeled thanks to a PV-based self-labeling focused on regions where the source and target marginal distributions are closer. Secondly, we propose an original process for tuning the hyperparameters. Our framework shows very promising results on a toy problem.

==> entete.tex <==
\RequirePackage{amsmath, amsfonts,amssymb, amsthm}



\newcommand\textm[1]{{\cursive #1}}
\newcommand\mathm[1]{\text{\cursive #1}}
%\newcommand{\Hilbert}{{\footnotesize \mathm{H}}\,}
\newcommand{\Hilbert}{\Hcal}

\newcommand{\Dcal}{{\cal D}}
\newcommand{\Id}{{\bf Id}}
\newcommand{\Ibf}{{\bf I}}

\newcommand{\iter}{\mathm{it}}
\newcommand{\frec}{\mathcal{R}}
\newcommand{\fcomp}{\mathcal{C}}

\newcommand{\reg}{\operatorname{reg}}

\newcommand{\supp}{\operatorname{supp}}
\newcommand{\pen}{\operatorname{pen}}

\newcommand{\dist}{\operatorname{\mathm{d}}}
\newcommand{\des}{\operatorname{dis}_\posterior}
\newcommand{\desw}{\operatorname{dis}_{\posterior_{\alphabf'}}}

\newcommand{\dive}{\operatorname{div}}
\newcommand{\VC}{\operatorname{VC}}

\newcommand{\chapeau}[1]{\hat{#1}}

\newcommand{\degree}{^{\circ}}
\newcommand{\nbpi}{\mbox{\scriptsize $\Pi$}}

\newcommand{\egt}{$(\epsilon,\!\gamma,\!\tau)$}

\newcommand{\xbs}{\mathbf{x}^s}
\newcommand{\xbt}{\mathbf{x}^t}
\newcommand{\Mbf}{\mathbf{M}}
\newcommand{\mbf}{\mathbf{m}}
\newcommand{\Abf}{\mathbf{A}}
%\newcommand{\wbf}{\mathbf{w}}
\newcommand{\ubf}{\mathbf{u}}
\newcommand{\vbf}{\mathbf{v}}

\newcommand{\xbfs}{\mathbf{x}^s}
\newcommand{\xbft}{\mathbf{x}^t}
\newcommand{\ys}{y^s}
\newcommand{\yt}{y^t}
\newcommand{\ms}{m^s}
\newcommand{\mt}{m^t}

\newcommand{\mun}{m_u}

\newcommand{\msu}{m_u^s}
\newcommand{\mtu}{m_u^t}

\newcommand{\mus}{\msu}
\newcommand{\mut}{\mtu}

\newcommand{\xs}{\xbfs}
\newcommand{\xt}{\xbft}

\newcommand{\SU}{S_u}
\newcommand{\TU}{T_u}

\newcommand{\Su}{\SU}
\newcommand{\Tu}{\TU}




\newcommand{\xbf}{\mathbf{x}}
\newcommand{\xb}{\xbf}
\newcommand{\wbf}{\mathbf{w}}

\newcommand{\ex}{(\xbf,y)}
\newcommand{\Y}{Y}
\newcommand{\X}{X}


%\newcommand{\Abf}{\mathbf{A}}
\newcommand{\Bbf}{\mathbf{B}}
\newcommand{\Cbf}{\mathbf{C}}
\newcommand{\Dbf}{\mathbf{D}}
\newcommand{\alphabf}{\boldsymbol{\alpha}}
\newcommand{\hdh}{\Hcal}
\newcommand\rouge[1]{\textcolor{red}{#1}}

\newcommand{\dilatation}{\mathcal{D}}
\newcommand{\I}{\mathrm{\bf I}}
\newcommand{\indicator}[1]{\I\left(#1\right)}

\newcommand{\leqo}{\preccurlyeq}

%\nomenclature{$\I(a)$}{Fonction indicatrice : renvoit $1$ si $a$ est vraie, $0$ sinon.}

\newcommand{\Jbf}{\mathbf{I}}
\newcommand{\jbf}{\mathbf{i}}
\newcommand{\jbfmax}{\jbf_{\max}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\Risk}{\mathbf{R}}
\newcommand{\Rbayes}{\Risk_{bayes}}

\newcommand{\GQ}{G_{\posterior}}
\newcommand{\BQ}{B_{\posterior}}
\newcommand{\GQstar}{G_{\posterior_t^*}}

\newcommand{\expo}[1]{
%    \mathrm{e}^{#1}
\exp\left(#1\right)
}

\newcommand{\expobis}[1]{
   \mathrm{e}^{#1}
%\exp\left(#1\right)
}

\newcommand{\transpoz}[1]{{#1}^{\top}}

\newcommand{\SPS}{S_{P_S}}
\newcommand{\SPSX}{S_{{P_S}|X}}
\newcommand{\PS}{P_S}
\newcommand{\PT}{P_T}
\newcommand{\DS}{D_S}
\newcommand{\DT}{D_T}
\newcommand{\DY}{D_Y}
\newcommand{\PThat}{\widehat{P_T}}

\newcommand{\RPThat}{\Risk_{\PThat}}
\newcommand{\RThat}{\Risk_{\widehat{T}}}

\newcommand{\SPT}{S_{P_T}}
\newcommand{\RPS}{\Risk_{P_S}}
\newcommand{\RPT}{\Risk_{P_T}}
\newcommand{\RDS}{\Risk_{D_S}}
\newcommand{\RDT}{\Risk_{D_T}}

\newcommand{\RT}{\Risk_{T}}
\newcommand{\RP}{\Risk_{P}}
\newcommand{\RD}{\Risk_{D}}

\newcommand{\RS}{\Risk_{S}}

\newcommand{\RSU}{\Risk_{\SU}}
\newcommand{\RTU}{\Risk_{\TU}}
\newcommand{\RSkappa}{\hat{\Risk}_{\kappa}}
\newcommand{\Rkappa}{\Risk_{\kappa}}
\newcommand{\RSPS}{\RS} %isk_{\SPS}}
\newcommand{\RSPT}{\RT} %Risk_{\SPT}}
\newcommand{\RST}{\Risk_{{(S,T)}}}

\newcommand{\DST}{{\DS\!\times\!\DT}}
\newcommand{\ST}{{S\!\times\! T}}
\newcommand{\RDSTa}{{\Risk_{{\DST}}^{(1)}}}
\newcommand{\RSTa}{{\Risk_{{S\!\times\!T}}^{(1)}}}

\newcommand{\x}{\times}

\newcommand{\Fcal}{\mathcal{F}}

\newcommand{\zo}{0\!-\!1}
\newcommand{\couples}{{\cal C}}
\newcommand{\paires}{\couples}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\loss}{\ell}
\newcommand{\losslin}{\loss_{lin}}

\newcommand{\lossO}{\loss_{\zo}}
\newcommand{\hingeloss}{\ell_{h\!i\!n\!g\!e}\!}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\lossPhi}{\loss_{\Erf}}

\newcommand{\oloss}[2]{\loss_{#1}^{\,\posterior}(\omega#2)}
\newcommand{\olosso}[3]{\loss_{#1}^{\,\posterior}(#3#2)}


\newcommand{\Loss}{\Risk} %\mathcal{L}}
\newcommand{\LossD}{\Loss_{D}}

\newcommand{\LossP}{\Loss_{P}}
\newcommand{\LossS}{\Loss_{S}}
\newcommand{\LossPl}{\LossP^{\loss}}
\newcommand{\LossSl}{\LossS^{\loss}}
\newcommand{\LossSU}{\Loss_{\SU}}

%\newcommand{\RPloss}{R_{P}^{\loss}}
%\newcommand{\EPloss}{\esp{}\!_{P}^{\loss}}

\newcommand{\som}[2]{\sum_{#1}^{#2}}

\newcommand{\argmax}[1]{
    \underset{#1}{\mathrm{argmax}}\
}
\newcommand{\argmin}[1]{
    \underset{#1}{\mathrm{argmin}}\
}

\newcommand{\argmindevant}[1]{
    {\mathrm{argmin}}_{#1}\
}

\newcommand{\prob}[1]{
    \underset{#1}{\mathrm{\bf Pr}}\
}
\newcommand{\probdevant}[1]{
    \mathrm{\bf Pr}_{#1}\
}

\newcommand{\Prob}[1]{\prob{#1}}
\renewcommand{\Pr}[1]{\prob{#1}}

\newcommand{\esp}[1]{
    \underset{#1}{\mathrm{\bf E}}\
}


\newcommand{\supr}[1]{
    \underset{#1}{\sup}\
}


\newcommand{\espdevant}[1]{
    \mathrm{\mathrm{\bf E}}_{#1}\,
}

%\newcommand{\var}[1]{
%    \underset{#1}{{\rm\bf Var}}\
%}
%\newcommand{\vari}[1]{
%    \underset{#1}{\mathrm{VAR}}\
%}
\newcommand{\var}[1]{
    \underset{#1}{\rm\bf Var}\
}
\newcommand{\vardevant}[1]{
    \mathrm{\rm\bf Var}_{#1}\,
}
\newcommand{\espcarre}[1]{
    \underset{#1}{\mathrm{\Eb^2}}\
} 

\newcommand{\LB}{\left[}
\newcommand{\RB}{\right]}

\newcommand{\diag}{\operatorname{diag}}
\newcommand{\dimension}{\operatorname{dim}}

\newcommand{\sign}{\operatorname{sign}}
\newcommand{\kl}{\operatorname{kl}}
\newcommand{\KL}{\operatorname{KL}}

\newcommand{\posterior}{\rho}
\newcommand{\prior}{\pi}
\newcommand{\PRIOR}{\boldsymbol{\prior}}
\newcommand{\POSTERIOR}{\boldsymbol{\posterior}}

\newcommand{\Qfrak}{\posterior}
\newcommand{\Pfrak}{\prior}

%\newcommand{\egaldef}{\ \stackrel{def}{=}\ }
\newcommand{\egaldef}{=}
\newcommand{\eqdef}{\egaldef}
\newcommand{\disc}{\operatorname{disc}}


\newcommand{\Erf}{\ensuremath{\textbf{Erf}}}

\newcommand{\phib}{\pmb{\phi}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\Kbf}{\mathbf{K}}

\newcommand{\Phidis}{\loss_{\rm dis}}
\newcommand{\lossPhic}{\loss_{\Erf_{\rm cvx}}}
\newcommand{\Phic}{\lossPhic}


\newcommand{\Scal}{\mathcal{S}}

\newcommand{\gc}[2]{\esp{h\sim \posterior}\I(h(#1)=#2)}



\newcommand{\MQ}{\M{}{\posterior}}
\newcommand{\MQP}{\M{P}{\posterior}}
\newcommand{\MQS}{\M{S}{\posterior}}
\newcommand{\MQSdeux}{\M{S}{\posterior^2}}

%\newcommand{\MQD}[1]{\M{D}{\posterior}}
\newcommand{\MQPdeux}{\M{P}{\posterior^2}}
%\newcommand{\MQD}[1]{\M{D}{\posterior}}

\newcommand{\M}[2]{\mathcal{M}^{#2}_{#1}}
\newcommand{\MS}[1]{\M{S}{#1}}
\newcommand{\MP}[1]{\M{P}{#1}}
\newcommand{\MD}[1]{\M{D}{#1}}



\newcommand{\mqdeux}[1]{\M{#1}{\posterior^2}}
\newcommand{\mmq}[1]{\M{#1}{\posterior}}
\newcommand{\mmqdeux}[1]{\M{#1}{\posterior^2}}
\newcommand{\mq}[1]{\M{#1}{\posterior}}
\newcommand{\mmodeux}[1]{\mmqdeux{#1}}
\newcommand{\mmo}[1]{\mmq{#1}}

\newcommand{\sq}[1]{\Scal_{#1}^{\posterior}}
\newcommand{\sqdeux}[1]{\Scal_{#1}^{\posterior^2}}

\newcommand{\ssq}[1]{\Scal_{#1}^{\posterior}}
\newcommand{\ssqdeux}[1]{\Scal_{#1}^{\posterior^2}}



\newcommand{\Cborne}{C^{\,\posterior}_P}
\newcommand{\CborneS}{C^{\,\posterior}_S}

\newcommand{\Fborne}{F^{\,\posterior}_P}
\newcommand{\FborneS}{F^{\,\posterior}_S}

\newcommand{\Oborne}{\Omega^{\,\posterior}_P}
\newcommand{\OborneS}{\Omega^{\,\posterior}_S}


